Copula for Instance-wise Feature Selection and Ranking

Instance-wise feature selection and ranking methods can achieve a good selection of task-friendly features for each sample in the context of neural networks. However, existing approaches that assume feature subsets to be independent are imperfect when considering the dependency between features. To address this limitation, we propose to incorporate the Gaussian copula, a powerful mathematical technique for capturing correlations between variables, into the current feature selection framework with no additional changes needed. Experimental results on both synthetic and real datasets, in terms of performance comparison and interpretability, demonstrate that our method is capable of capturing meaningful correlations.

==> UAI2023/algo3.tex <==
 
 \begin{algorithm}[t]
\caption{Sampling Scheme via Top-$k$ Ranking.}
\label{algo:sample_topk_ranking}
\KwIn{Feature vector $\boldsymbol{x} \in \mathbb{R}^{d}$ with its corresponding weight $\boldsymbol{\alpha} \in \mathbb{R}^{d}$, full-rank or low-rank matrix $\boldsymbol L$ and noise level $\sigma^2$, identity matrix $\boldsymbol{I}$, tuning parameter $t,\delta$. }
\KwOut{Binary mask vector $\boldsymbol{z} \in \{0,1\}^d$.}
Apply Algorithm~\ref{algo:corr_noise} to obtain correlated noise vector $\boldsymbol u$\;

Compute keys $v_i = u_i^{1 / \alpha_i},$ $\forall i=2,\ldots,d$,$v_1 = u_1$;

Take the log transformation $\log(\cdot)$ to $v_i$, and rewrite the key $ v_i=(1 / \alpha_i) \log(u_i)$\;

\For{$s\gets 2$ \KwTo $k$ }{
   ${v}_i^{s} = {v}_i^{s-1} + t^{\delta} \log(1 - p_i^{s-1}), \forall i=1,\ldots,d$ \;
   
   $p_i^s = \frac{\exp\{{v}_i^s/t\}}{\sum_{l=1}^d \exp\{{v}_l^s/t\}}, \forall i=1,\ldots,d$\
    }
$\boldsymbol{\tilde z} = \sum_{s=1}^k  \boldsymbol p^s$\;

Obtain feature indicator vector $\boldsymbol z$ via masking the top-$k$ largest elements in $\boldsymbol {\tilde z}$ with 1, other elements with 0 \;
\end{algorithm}
